Privacy Partitioning: Protecting User Data During the Deep Learning Inference Phase

We present a practical method for protecting data during the inference phase of deep learning based on bipartite topology threat modeling and an interactive adversarial deep network construction. We term this approach \emph{Privacy Partitioning}. In the proposed framework, we split the machine learning models and deploy a few layers into users' local devices, and the rest of the layers into a remote server. We propose an approach to protect user's data during the inference phase, while still achieve good classification accuracy. We conduct an experimental evaluation of this approach on benchmark datasets of three computer vision tasks. The experimental results indicate that this approach can be used to significantly attenuate the capacity for an adversary with access to the state-of-the-art deep network's intermediate states to learn privacy-sensitive inputs to the network. For example, we demonstrate that our approach can prevent attackers from inferring the private attributes such as gender from the Face image dataset without sacrificing the classification accuracy of the original machine learning task such as Face Identification.

==> sections/00-acknowledgment.tex <==
% Acknowledgements 

The authors would like to thank members of the INI Privacy-Preserving Machine Learning team--Yiming Liu, Swee Sim, Haodong Liu, Vibha Iyengar, and  Jiasen Chen--for their valuable contributions to 
completing this work, and the anonymous reviewers for their detailed comments and valuable feedback.
